Deep Optimized Priors for 3D Shape Modeling and Reconstruction

Many learning-based approaches have difficulty scaling to unseen data, as the generality of its learned prior is limited to the scale and variations of the training samples. This holds particularly true with 3D learning tasks, given the sparsity of 3D datasets available. We introduce a new learning framework for 3D modeling and reconstruction that greatly improves the generalization ability of a deep generator. Our approach strives to connect the good ends of both learning-based and optimization-based methods. In particular, unlike the common practice that fixes the pre-trained priors at test time, we propose to further optimize the learned prior and latent code according to the input physical measurements after the training. We show that the proposed strategy effectively breaks the barriers constrained by the pre-trained priors and could lead to high-quality adaptation to unseen data. We realize our framework using the implicit surface representation and validate the efficacy of our approach in a variety of challenging tasks that take highly sparse or collapsed observations as input. Experimental results show that our approach compares favorably with the state-of-the-art methods in terms of both generality and accuracy.

==> sections/Bak/method_inference.tex <==
\subsection{Inference Process}
During inference process, a sparse observation $\mathcal{X}$ is given for an object $\mathcal{S}$, and the goal is to reconstruct $\mathcal{S}$ specifically.
In the existing work \cite{}, $\bm{z}$ is optimized via Maximum-a-Posterior (MAP) estimation, with the categorical prior fixed.
However, such learnt prior are extremely limited by the training data, which could hardly apply to all the situations, especially when there exists a gap between the training data and the test data.
Therefore, in this section, we introduce a new framework that optimizing both the latent shape-code of $\bm{z}$ and categorical prior of $\bm{\theta}$.

First of all, prior learnt from the training data should be robust enough during the optimization.
In other words, we expect a flat, invariant region around the well-optimized $\bm{\theta}$.
This is why we introduce hypernetwork, whose parameters could be relatively fewer comparing to the parameters of using the implicit neural networks to learn the categorical prior directly, as shown in \cite{ha2016hypernetworks}.
With lower dimensional parameters, the problem of curse of dimensionality could be alleviated, leading to a  more concentrated parameter space and more compact shape manifold.
This is the precondition for us to fine-tuning the categorical prior of $\bm{\theta}$ during inference process.

Then, even though the categorical prior region we learnt are relatively robust, we can hardly expect the optimization to be perfectly proper, since the observations are sparse.
Without additional constrain, the categorical prior could still easily slide into the wrong area, which making the prior futile and resulting in a strange shape.
Therefore, when optimizing $\theta$ during inference process, we should prevent $\theta$ from moving too far from the learnt categorical prior $\bm{\theta}_0$.
To achieve this, we introduce another loss of prior consistency loss, which can simply be defined as
\begin{equation}\label{eq:PriorConsistLoss}
  \mathcal{L}_{Prior}(\bm{\theta}) = \|\bm{\theta} - \bm{\theta}_0\|_2^2.
\end{equation}
Such loss is simple but effectiveness.

Overall, the loss used during the inference process is very similar to the one in Eq. (\ref{eq:TrainingLoss}), with an additional loss in Eq. (\ref{eq:PriorConsistLoss}), which can be defined as
\begin{equation}\label{eq:InferenceLoss}
  \mathcal{L}_{Inference}(\mathcal{X}, \bm{z}, \bm{\theta}) =  \mathcal{L}_{Training}(\mathcal{X}, \bm{z}, \bm{\theta}) + \lambda_4 \mathcal{L}_{Prior}(\bm{\theta}),
\end{equation}
where $\lambda_4$ is also the penalty parameters, whose default value is set as $\lambda_4 = $.

==> sections/Bak/method_training.tex <==
\subsection{Training Process}
The goal of training process is to learn the categorical prior for $\theta$ in the hypernetwork $h$, and to construct the latent shape-code space.
With the components mentioned above, especially the differentiable renderer, the objective of Eq. (\ref{eq:OverallObjective}) can be reformulated as
\begin{equation}\label{eq:ourObjective}
    \min_{\bm{\theta}, \bm{z}} \mathbb{E}
_{\bm{I_i}\in\mathcal{I}} [\hat{D}(\bm{I}_i, \hat{\bm{I}}(\bm{P}_i, \bm{K}_i; f_{h_{\bm{\theta}}(\bm{z})}, g_{h_{\bm{\theta}}(\bm{z})}))],
\end{equation}
where $\hat{\bm{I}}$ denotes the differentiable rendering, $\hat{D}$ denotes the distance between two images, and the other notations are consistent with the ones above.
In the following section, without introducing ambiguity, we abbreviate $\hat{\bm{I}}(\bm{P}_i, \bm{K}_i; f_{h_{\bm{\theta}}(\bm{z})}, g_{h_{\bm{\theta}}(\bm{z})})$ as $\hat{\bm{I}}_i$.

\noindent\textbf{RGB Loss --}
For the pixels in the given image, we divide them into two sets, of which one is those located inside the mask $\bm{M}$, denoted as $\mathcal{P}_1 = \{p | p\in\bm{M} \cap \hat{\bm{M}}\}$, $\hat{\bm{M}}$ is the mask predicted from our generated shape, which follows \cite{yariv2020multiview}.
The RGB loss can be formally defined as
\begin{equation}\label{eq:rgbLoss}
    \mathcal{L}_{RGB}(\mathcal{X}, \bm{\theta}) = \sum_{i} \sum_{p\in\mathcal{P}_1} \|\bm{I}_i(p) - \hat{\bm{I}}_i(p) \|_1.
\end{equation}

\noindent\textbf{Mask Loss --}
The mask loss is also part of $\hat{D}$, measuring the silhouette between the given surface and our generated surface.
We adopt mask loss since RGB loss could achieve its minima via shrinking $\hat{\bm{M}}$ to be zero.
Therefore, mask loss here is to prevent the eliminate of $\hat{\bm{M}}$.
Mask loss can be formally defined as
\begin{equation}\label{eq:maskLoss}
    \mathcal{L}_{Mask}(\mathcal{X}, \bm{\theta}) = \sum_{i} \sum_{p\in\bm{I}_i} CE(\bm{M}_i(p), \hat{\bm{M}}_i(p)),
\end{equation}
where $CE$ is cross entropy loss.

\noindent\textbf{Normal Loss --}
We also take the smooth prior that the normals within a surface patch should point to the similar directions.
Normal loss can be formally defined as
\begin{equation}\label{eq:normalLoss}
    \mathcal{L}_{Normal}(\mathcal{X}, \bm{\theta}) = \sum_{\bm{x}_j\in\bm{S}}( \bm{n}(\bm{x_j}) -  \frac{1}{k}\sum_{\bm{x}\in\mathcal{N}_{\bm{x}_j}} \bm{n}(\bm{x})),
\end{equation}
where $\bm{n}$ is the estimated normal follows \cite{DVR}, $\mathcal{N}_{\bm{x}_j}$ is a $k$ nearest neighbors points for point $\bm{x}_j$.

\noindent\textbf{Gaussian Prior Loss --}
As mentioned above, we assume the prior distribution of the latent shape-code to be be a zero-mean multivariate-Gaussian with a spherical covariance $\sigma^2 I$.
And we achieve this via the Gaussian prior loss,
\begin{equation}\label{eq:GaussianLoss}
    \mathcal{L}_{Gaussian}(\bm{z}) = \|\bm{z}\|_2^2.
\end{equation}

\noindent\textbf{The Combined Objective --} We use the following combined objective to learn the categorical prior for $\theta$ in the hypernetwork $h$, and to construct the latent shape-code space
\begin{equation}\label{eq:TrainingLoss}
    \begin{split}
      \mathcal{L}_{Training}(\mathcal{X}, \bm{z}, &\bm{\theta}) =  \mathcal{L}_{RGB}(\mathcal{X}, \bm{\theta}) + \lambda_1\cdot\mathcal{L}_{Mask}(\mathcal{X}, \bm{\theta}) + \\
      & \lambda_2\cdot\mathcal{L}_{Normal}(\mathcal{X}, \bm{\theta}) + \lambda_3\cdot\mathcal{L}_{Gaussian}(\bm{z}),
    \end{split}
\end{equation}
where $\lambda_1$, $\lambda_2$ and $\lambda_3$ are penalty parameters whose default values are set as $\lambda_1=$, $\lambda_2=$, $\lambda_3=$, which work well in all our experiments.
The combined objective $\mathcal{L}(\mathcal{X}, z)$ is perform on the additional dataset $\{\mathcal{X}^j\}_{j=1}^M$, where dense views are provided for each $\mathcal{X}\in\{\mathcal{X}^j\}$ to make the learning feasible.
